Analyzing Wage Theft in Day Labor Markets via Principal Agent Models

In day labor markets, workers are particularly vulnerable to wage theft. This paper introduces a principal-agent model to analyze the conditions required to mitigate wage theft through fines and establishes the necessary and sufficient conditions to reduce theft. We find that the fines necessary to eliminate theft are significantly larger than those imposed by current labor laws, making wage theft likely to persist under penalty-based methods alone. Through numerical analysis, we show how wage theft disproportionately affects workers with lower reservation utilities and observe that workers with similar reservation utilities experience comparable impacts, regardless of their skill levels. To address the limitations of penalty-based approaches, we extend the model to a dynamic game incorporating worker awareness. We prove that wage theft can be fully eliminated if workers accurately predict theft using historical data and employers follow optimal fixed wage strategy. Additionally, sharing wage theft information becomes an effective long-term solution when employers use any given fixed wage strategies, emphasizing the importance of raising worker awareness through various channels.

==> OptimalValuesForWAsFunctionOFEffortAndTheft.tex <==
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}[xscale=5,yscale=1.2]
        %\draw[->] (0, 0) -- (1.1, 0) node[right] {$\a$};
      %\draw[->] (0, 0) -- (0, 6.5);
      %\draw[scale=0.5, domain=-3:3, smooth, variable=\x, blue] plot ({\x}, {\x*\x});
      
      %%%%%%%%%%%%W_L for C(a)=a^3+a^2+a and u=0.5
      \draw[domain=0:0.5, smooth,  thick, variable=\x, blue] plot ({\x}, {0.5-2*\x*\x*\x-\x*\x});
      \draw[domain=0.5:1, smooth,  thick, variable=\x, blue] plot ({\x}, 0);
      
      %%%%%%%%%%%%W_h
      \draw[domain=0:0.5, smooth,  thick, variable=\x, red] plot ({\x}, {0.5-2*\x*\x*\x+2*\x*\x+2*\x+1});
      \draw[domain=0.5:1, smooth,  thick, variable=\x, red] plot ({\x}, 3*\x*\x+2*\x+1);
      
      %%%%%Lines that tell us things
      
        %%%%%vertical lines
        %\draw[dashed] (0.5,6)--(0.5,0) node[below] {$\bar{u}-\a\cdot \c (\a) + \C (\a)=0$};
        \draw[dashed] (1,6)--(1,0) node[below left] {$\a=1$};
        \draw[dashed] (0,6)--(0,0) node[below right] {$\a=0$};
      
        %%%%%horizontal lines
        \draw[dashed] (0,0)--(1,0);
        
        %%%%%%%%%%%%%%%%%%%%%%%%        %%%%%%%%%%%%%%%%%%%%%%%%        %%%%%%%%%%%%%%%%%%%%%%%%
        \draw[dashed] (1,6)--(0,6) node[midway, above] {$\beta \in (0, \bar{u}]$}; 
        %\draw[dashed] (1,0.5)--(0,0.5);
        %\draw[dashed] (1,1.5)--(0,1.5);
      
        %%%%\c (\a) lines
        %\draw[thick, <->] (0.75,4.188) -- (0.75,0) node[midway, right] {$\c (\a)$};
        %\draw[thick, <->] (0.25,.406) -- (0.25,2.094) node[midway, right] {$\c (\a)$};
      
      
      
      %%%%%%%%%%B_L/B_H
      \draw[dotted] (0,0.25)--(1,0.25) node[above left] {$\beta : \P'(\beta)=1$};
      
      
      %b_H
      \draw[dashed, ultra thick, violet] (0,0.25)--(1,0.25);
      
      %b_L
      \draw[domain=0:.3774, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, 0.25);
      \draw[domain=0.3774:0.5, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, {0.5-2*\x*\x*\x-\x*\x});
      \draw[domain=0.5:1, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, 0);
      
      
      %%%%%%%Legend
      \draw[thick] (0.025, 5.75)--(0.025, 4.125)--(0.725,4.125)--(0.725,5.75)--cycle;
      
      \draw[thick, blue] (0.05,5.5)--(0.1,5.5) node[right, blue] {$w_L$};
      \draw[thick, red] (0.05,5.125)--(0.1,5.125) node[right, red] {$w_H$};
      \draw[ultra thick, dashed, violet] (0.05,4.75)--(0.1,4.75) node[right, violet] {$b_H=\min\{\beta,w_H\}$};
      \draw[ultra thick, dashed, orange] (0.05,4.375)--(0.1,4.375) node[right, orange] {$b_L=\min\{\beta,w_L\}$};
      
    \end{tikzpicture}
    \hfill
    \begin{tikzpicture}[xscale=5,yscale=1.2]
        %\draw[->] (0, 0) -- (1.1, 0) node[right] {$\a$};
      %\draw[->] (0, 0) -- (0, 6.5);
      %\draw[scale=0.5, domain=-3:3, smooth, variable=\x, blue] plot ({\x}, {\x*\x});
      
      %%%%%%%%%%%%W_L for C(a)=a^3+a^2+a and u=0.5
      \draw[domain=0:0.5, smooth,  thick, variable=\x, blue] plot ({\x}, {0.5-2*\x*\x*\x-\x*\x});
      \draw[domain=0.5:1, smooth,  thick, variable=\x, blue] plot ({\x}, 0);
      
      %%%%%%%%%%%%W_h
      \draw[domain=0:0.5, smooth,  thick, variable=\x, red] plot ({\x}, {0.5-2*\x*\x*\x+2*\x*\x+2*\x+1});
      \draw[domain=0.5:1, smooth,  thick, variable=\x, red] plot ({\x}, 3*\x*\x+2*\x+1);
      
      %%%%%Lines that tell us things
      
        %%%%%vertical lines
        %\draw[dashed] (0.5,6)--(0.5,0) node[below] {$\bar{u}-\a\cdot \c (\a) + \C (\a)=0$};
        \draw[dashed] (1,6)--(1,0) node[below left] {$\a=1$};
        \draw[dashed] (0,6)--(0,0) node[below right] {$\a=0$};
      
        %%%%%horizontal lines
        \draw[dashed] (0,0)--(1,0);
        
                %%%%%%%%%%%%%%%%%%%%%%%%        %%%%%%%%%%%%%%%%%%%%%%%%        %%%%%%%%%%%%%%%%%%%%%%%%
        \draw[dashed] (1,6)--(0,6) node[midway, above] {$\beta \in [\bar{u}, \bar{u} + \c(0)]$};
        %\draw[dashed] (1,0.5)--(0,0.5);
        %\draw[dashed] (1,1.5)--(0,1.5);
      
        %%%%\c (\a) lines
        %\draw[thick, <->] (0.75,4.188) -- (0.75,0) node[midway, right] {$\c (\a)$};
        %\draw[thick, <->] (0.25,.406) -- (0.25,2.094) node[midway, right] {$\c (\a)$};
      
      
      
      %%%%%%%%%%B_L/B_H
      \draw[dotted] (1,1)--(0,1) node[midway, above] {$\beta : \P'(\beta)=1$};
      \draw[dashed, ultra thick, violet] (1,1)--(0,1);
      
      
      \draw[domain=0:0.5, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, {0.5-2*\x*\x*\x-\x*\x});
      \draw[domain=0.5:1, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, 0);
      
      
      %%%%%%%Legend
      \draw[thick] (0.025, 5.75)--(0.025, 4.125)--(0.725,4.125)--(0.725,5.75)--cycle;
      
      \draw[thick, blue] (0.05,5.5)--(0.1,5.5) node[right, blue] {$w_L$};
      \draw[thick, red] (0.05,5.125)--(0.1,5.125) node[right, red] {$w_H$};
      \draw[ultra thick, dashed, violet] (0.05,4.75)--(0.1,4.75) node[right, violet] {$b_H=\min\{\beta,w_H\}$};
      \draw[ultra thick, dashed, orange] (0.05,4.375)--(0.1,4.375) node[right, orange] {$b_L=\min\{\beta,w_L\}$};
      
    \end{tikzpicture}
    \hfill
    \begin{tikzpicture}[xscale=5,yscale=1.2]
        %\draw[->] (0, 0) -- (1.1, 0) node[right] {$\a$};
      %\draw[->] (0, 0) -- (0, 6.5);
      %\draw[scale=0.5, domain=-3:3, smooth, variable=\x, blue] plot ({\x}, {\x*\x});
      
      %%%%%%%%%%%%W_L for C(a)=a^3+a^2+a and u=0.5
      \draw[domain=0:0.5, smooth,  thick, variable=\x, blue] plot ({\x}, {0.5-2*\x*\x*\x-\x*\x});
      \draw[domain=0.5:1, smooth,  thick, variable=\x, blue] plot ({\x}, 0);
      
      %%%%%%%%%%%%W_h
      \draw[domain=0:0.5, smooth,  thick, variable=\x, red] plot ({\x}, {0.5-2*\x*\x*\x+2*\x*\x+2*\x+1});
      \draw[domain=0.5:1, smooth,  thick, variable=\x, red] plot ({\x}, 3*\x*\x+2*\x+1);
      
      %%%%%Lines that tell us things
      
        %%%%%vertical lines
        %\draw[dashed] (0.5,6)--(0.5,0) node[below] {$\bar{u}-\a\cdot \c (\a) + \C (\a)=0$};
        \draw[dashed] (1,6)--(1,0) node[below left] {$\a=1$};
        \draw[dashed] (0,6)--(0,0) node[below right] {$\a=0$};
      
        %%%%%horizontal lines
        \draw[dashed] (0,0)--(1,0);
        \draw[dashed] (1,6)--(0,6) node[midway, above] {$\beta \in [\bar{u}+\c(0), \infty)$}; 
        %\draw[dashed] (1,0.5)--(0,0.5);
        %\draw[dashed] (1,1.5)--(0,1.5);
      
        %%%%\c (\a) lines
        %\draw[thick, <->] (0.75,4.188) --https://www.overleaf.com/project/622150b2ad0a84d58257541c (0.75,0) node[midway, right] {$\c (\a)$};
        %\draw[thick, <->] (0.25,.406) -- (0.25,2.094) node[midway, right] {$\c (\a)$};
      
      
      
      %%%%%%%%%%B_L/B_H
      \draw[dotted] (1,3.87)--(0,3.87) node[below right] {$\beta : \P'(\beta)=1$};
      
      
      %%%%%b_H


      
      \draw[dashed, ultra thick, violet] (1,3.87)--(0.7,3.87);
      \draw[domain=0:0.5, smooth, ultra thick, variable=\x, violet,dashed] plot ({\x}, {0.5-2*\x*\x*\x+2*\x*\x+2*\x+1});
      \draw[domain=0.5:0.7, smooth, ultra thick, variable=\x, violet, dashed] plot ({\x}, 3*\x*\x+2*\x+1);      
      
      \draw[domain=0:0.5, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, {0.5-2*\x*\x*\x-\x*\x});
      \draw[domain=0.5:1, smooth, dashed, ultra thick, variable=\x, orange] plot ({\x}, 0);
      
      
      %%%%%%%Legend
      \draw[thick] (0.025, 5.75)--(0.025, 4.125)--(0.725,4.125)--(0.725,5.75)--cycle;
      
      \draw[thick, blue] (0.05,5.5)--(0.1,5.5) node[right, blue] {$w_L$};
      \draw[thick, red] (0.05,5.125)--(0.1,5.125) node[right, red] {$w_H$};
      \draw[ultra thick, dashed, violet] (0.05,4.75)--(0.1,4.75) node[right, violet] {$b_H=\min\{\beta,w_H\}$};
      \draw[ultra thick, dashed, orange] (0.05,4.375)--(0.1,4.375) node[right, orange] {$b_L=\min\{\beta,w_L\}$};
      
    \end{tikzpicture}
    \caption{Optimal values for $b_H$ and $b_L$ as functions of effort $\a$ and ideal theft $\beta$ (Lemmas \ref{lem:IdealTheft} and \ref{lem:OptConditions}).} \label{fig:bHbL}
\end{figure}

